Twitter and Polls: Analyzing and estimating political orientation of Twitter users in India General #Elections2014

This year (2014) in the month of May, the tenure of the 15th Lok Sabha was to end and the elections to the 543 parliamentary seats were to be held. A whooping $5 billion were spent on these elections, which made us stand second only to the US Presidential elections in terms of money spent. Swelling number of Internet users and Online Social Media (OSM) users could effect 3-4% of urban population votes as per a report of IAMAI (Internet & Mobile Association of India). Our count of tweets related to elections from September 2013 to May 2014, was close to 18.21 million. We analyzed the complete dataset and found that the activity on Twitter peaked during important events. It was evident from our data that the political behavior of the politicians affected their followers count. Yet another aim of our work was to find an efficient way to classify the political orientation of the users on Twitter. We used four different techniques: two were based on the content of the tweets, one on the user based features and another based on community detection algorithm on the retweet and user mention networks. We found that the community detection algorithm worked best. We built a portal to show the analysis of the tweets of the last 24 hours. To the best of our knowledge, this is the first academic pursuit to analyze the elections data and classify the users in the India General Elections 2014.

==> M.Tech thesis/mtech_thesis_cover.tex <==


\def\addrone{Your address}
\def\addrtwo{Your city}

\def\degree{M.Tech. in Computer Science with Specialization in Data Engineering}


\def\submissiondate{June 06, 2014}

\def\supervisorone{Dr. Ponnurangam Kumarguru}


\def\supervisortwo{Dr. Vinayak Naik}


\def\supervisorthree{Dr. Ayesha Choudhary}

\thispagestyle{empty}

\begin{center}

{\LARGE \bf {Twitter and Polls: Analyzing and estimating political orientation of Twitter users in India General \#Elections2014  }

 }  
 \vspace{1in}
 
 {\Large{Student Name: Abhishek Bhola}} \\  
 \vspace{.1in} 
 IIIT-D-MTech-CS-DE-12-MT12031 \\

 June 06, 2014 \\
  
    \vspace{.6in}

  \vspace{.5in}

{Indraprastha Institute of Information Technology\\
New Delhi}

\vspace{.8in}  {\underline{Thesis Committee} \\ \supervisorone                ~(Chair) \\ \supervisortwo \\ \supervisorthree} \\ \vspace{.35in}


\vspace{.6in} {Submitted in partial fulfillment of the requirements \\for the Degree of M.Tech. in Computer Science, \\ with specialization in Data Engineering}

\vspace{.8in}

\copyright 2014 Abhishek Bhola  \\ All rights reserved \\
\vspace{.8in}


\end{center}




